The Shear TEsting Programme 2: Factors affecting high precision weak lensing analyses

The Shear TEsting Programme (STEP) is a collaborative project to improve the accuracy and reliability of weak lensing measurement, in preparation for the next generation of wide-field surveys. We review sixteen current and emerging shear measurement methods in a common language, and assess their performance by running them (blindly) on simulated images that contain a known shear signal. We determine the common features of algorithms that most successfully recover the input parameters. We achieve previously unattained discriminatory precision in our analysis, via a combination of more extensive simulations, and pairs of galaxy images that have been rotated with respect to each other, thus removing noise from their intrinsic ellipticities. The robustness of our simulation approach is also confirmed by testing the relative calibration of methods on real data. Weak lensing measurement has improved since the first STEP paper. Several methods now consistently achieve better than 2% precision, and are still being developed. However, the simulations can now distinguish all methods from perfect performance. Our main concern continues to be the potential for a multiplicative shear calibration bias: not least because this can not be internally calibrated with real data. We determine which galaxy populations are responsible and, by adjusting the simulated observing conditions, we also investigate the effects of instrumental and atmospheric parameters. We have isolated several previously unrecognised aspects of galaxy shape measurement, in which focussed development could provide further progress towards the sub-percent level of precision desired for future surveys. [ABRIDGED]

==> build <==
\rm Massey.ps
\rm Massey_NotForReview.tar.gz
tar cfv Massey_NotForReview.tar .
gzip Massey_NotForReview.tar
latex step2.tex ; latex step2.tex #; latex step2.tex
dvips -t a4 step2.dvi -o step2.ps
#dvipdf -t a4 step2.dvi step2.pdf
\rm step2.log
\rm step2.dvi
\rm step2.aux
mv step2.ps Massey.ps

